GraphNeT 2.0 -- A Deep Learning Library for Neutrino Telescopes

Neutrino telescopes, an extension of traditional multiwavelength astronomy, provide a complementary view of the universe using neutrinos. Differences in detector geometry and detection medium mean that improvements to reconstruction techniques made at one experiment are not readily applicable to another. Recently, deep learning has been shown to improve prediction speed and accuracy and offer indifference to detector geometry and detection medium, providing a unique opportunity for collaboration. This work introduces GraphNeT 2.0, an open-source, detector-agnostic deep learning library for neutrino telescopes and related experiments. GraphNeT enables inter-experimental collaboration on the use and development of advanced methods based on major deep learning paradigms like transformers, normalizing flows, graph neural networks, and more.

==> sections/data.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.38\textwidth]{figures/converter.png}
  \end{center}
  \caption{Illustration of the Reader/Writer structure of the DataConverter in GraphNeT. The reader is an experiment-specific module that parses experiment-specific files. Writers save the extracted data to a data format suitable for deep learning.}
  \label{fig:converter}
\end{wrapfigure}
GraphNeT contains data conversion functionality that allows users to export data in experiment-specific file formats to formats suitable for deep learning. 
The \texttt{DataConverter}, illustrated in Figure \ref{fig:converter}, is a modularized data converter that accepts a \texttt{FileReader} and a \texttt{FileWriter}. The \texttt{FileReader} is an experiments-specific module, written to be able to parse and extract data from a single file in a experiment-specific format. The \texttt{FileWriter} writes the contents of the file to a specific file format which may be used for training models in GraphNeT. The \texttt{DataConverter} facilitates the exchange of data between the two modules and is fully parallelized. Therefore, extending \texttt{DataConverter} to convert files from new neutrino telescopes or related experiments only requires implementing a new \texttt{FileReader} able to parse the files. Likewise, extending \texttt{DataConverter} to export to a new format suitable for deep learning, only requires adding a new \texttt{FileWriter}. This design choice significantly lowers the technical overhead associated with implementing support for new experiments into GraphNeT, and extending it to support future file formats.
